Multi-View Representation is What You Need for Point-Cloud Pre-Training

A promising direction for pre-training 3D point clouds is to leverage the massive amount of data in 2D, whereas the domain gap between 2D and 3D creates a fundamental challenge. This paper proposes a novel approach to point-cloud pre-training that learns 3D representations by leveraging pre-trained 2D networks. Different from the popular practice of predicting 2D features first and then obtaining 3D features through dimensionality lifting, our approach directly uses a 3D network for feature extraction. We train the 3D feature extraction network with the help of the novel 2D knowledge transfer loss, which enforces the 2D projections of the 3D feature to be consistent with the output of pre-trained 2D networks. To prevent the feature from discarding 3D signals, we introduce the multi-view consistency loss that additionally encourages the projected 2D feature representations to capture pixel-wise correspondences across different views. Such correspondences induce 3D geometry and effectively retain 3D features in the projected 2D features. Experimental results demonstrate that our pre-trained model can be successfully transferred to various downstream tasks, including 3D shape classification, part segmentation, 3D object detection, and semantic segmentation, achieving state-of-the-art performance.

==> algorithm/algorithm.tex <==
\begin{algorithm}
\caption{General framework of MVNet}
\begin{algorithmic}[1]
\State \textbf{Input:} RGB-D scan pairs with camera parameters $S = \{(I_1^{i}, D_1^{i}), (I_2^{i}, D_2^{i}), K^{i}, E_1^{i}, E_2^{i}\}$, feature encoding network $\mathcal{F}_e$, 2D knowledge transfer module $\mathcal{F}_{2d}$, multi-view consistency module $\mathcal{F}_m$.
\State \textbf{Ouput:} Pre-trained weights of feature encoding network $\mathcal{F}_e$

\For{$\{(I_1, D_1), (I_2, D_2), K, E_1, E_2\}$ \textbf{in} RGB-D scan pairs}
\State - Project $(I_1, D_1), (I_2, D_2)$ into 3D point cloud $P$ via camera parameters $K, E_1, E_2$.
\State - Extract per-point feature volume: $F_P = \mathcal{F}_e(P)$.
\State - Project the feature volume back onto the original views to generate 2D feature maps $F_1, F_2$
\State - Employ 2D knowledge transfer module with square $L_2$ loss: $\mathcal{L}_{2d} = \mathcal{F}_{2d}(I_i, F_i)$
\State - Employ multi-view consistency module with the correspondence loss: $\mathcal{L}_{m} = \mathcal{F}_m(F_1, F_2)$
\State - Compute the total loss $\mathcal{L} = \mathcal{L}_{2d} + \lambda \mathcal{L}_m$.
\State - Backprop: to update $\mathcal{F}_e, \mathcal{F}_{2d}, \mathcal{F}_m$ with loss $\mathcal{L}$.
\EndFor
\end{algorithmic}
\label{alg:mvnet}
\end{algorithm}

==> figures/supp_cotr_2.tex <==
\begin{figure}[h]
    \begin{center}
    \includegraphics[width=1\linewidth]{images/supp_cotr.pdf}
    \end{center}
    \caption{\textbf{Qualitative results of multi-view consistency module prediction.} Each element consists of two different view images. The query points and prediction points are visualized using the blue dot, and they are connected by the green line.}
    \label{Fig:supp_cotr}
\end{figure}

==> figures/supp_eff.tex <==
\begin{figure}[h]
    \begin{center}
    \includegraphics[width=1\linewidth]{images/label_eff.pdf}
    \end{center}
    \caption{\textbf{Illustration of Label efficiency training.} Our model is pre-trained on ScanNet and subsequently fine-tuned separately on both ScanNet and SUN RGBD. We take VoteNet as network architecture. During this fine-tuning process, we employ varying percentages of labeled training data. Demonstrating its efficacy, our pre-training model not only surpasses the performance of models trained from scratch but also achieves comparable results utilizing only 60\% of the labeled data.}
    \label{fig:eff}
\end{figure}

==> figures/supp_qual.tex <==
\begin{figure}[h]
    \begin{center}
    \includegraphics[width=\linewidth]{images/visualize-3.pdf}
    \end{center}
    \caption{\textbf{Qualitative results on S3DIS semantic segmentation task.} We compare our method with the second-best approach, SceneContext~\citep{hou2021exploring}.}
    \label{Fig:srnet}
\end{figure}

==> figures/supp_qual_2.tex <==
\begin{figure}[h]
    \begin{center}
    \includegraphics[width=\linewidth]{images/visualize_4.pdf}
    \end{center}
    \caption{\textbf{More qualitative results on S3DIS semantic segmentation task.} We compare our method with the second-best approach, SceneContext~\citep{hou2021exploring}.}
    \label{Fig:srnet}
\end{figure}

==> figures/supp_radar_chart.tex <==
\begin{figure}[h]
    \centering   
    \includegraphics[width=0.7\linewidth]{images/radar_chart_multi.pdf}
    %\caption{Our model (blue) achieves state-of-the-art performance across a broad range of tasks at both the scene and shape levels. The distance to the origin indicates the task result.}
    \label{fig:radar}
\end{figure}

==> figures/supp_srnet.tex <==
\begin{figure}[h]
    \begin{center}
    \includegraphics[width=1\linewidth]{images/sr-unet.pdf}
    \end{center}
    \caption{\textbf{Feature encoding network details.}}
    \label{Fig:srnet}
\end{figure}

==> tables/detection.tex <==
\begin{table*}[t]
\centering
    \caption{\small{\textbf{3D Object Detection Results.} We fine-tune our pre-trained model on ScanNetV2~\cite{dai2017scannet} and SUN-RGBD~\cite{song2015sun} validation sets using VoteNet~\cite{qi2019deep} and CAGroup3D~\cite{wang2022cagroup3d}. We show mean Average Precision~(mAP) across all semantic classes with 3D IoU thresholds of 0.25 and 0.5. Methods in the second section denote self-supervised methods.}}
    \label{tab:detection}
   \setlength\tabcolsep{9pt}% 调整列间距
    \begin{tabular}{lcccccc}
        \toprule
     \multirow{2}{*}{Method} & \multirow{2}{*}{SSL} & \multicolumn{2}{c}{ScanNet} & \multicolumn{2}{c}{SUN RGB-D} \\
        \cmidrule(lr){3-4}   \cmidrule(lr){5-6}  & 
       &  mAP@0.25 & mAP@0.5 & mAP@0.25 & mAP@0.5 \\
        \midrule
        VoteNet~\cite{qi2019deep} & - &  58.6 & 33.5 & 57.7 & 32.9 \\
        3D-MPA~\cite{engelmann20203d}& - & 64.2 & 49.2 & - & - \\
        MLCVNet~\cite{xie2020mlcvnet}& - & 64.5 & 41.4 & 59.8 & - \\
        %H3DNet~\cite{zhang2020h3dnet} & 67.2 & 48.1 & 60.1 & 39.0 \\
        BRNet~\cite{cheng2021back}& - & 66.1 & 50.9 & 61.1 & 43.7 \\
        3DETR~\cite{misra2021end}& - & 65.0 & 47.0 & 59.1 & 32.7 \\
        GroupFree~\cite{liu2021group}& - & 69.1 & 52.8 & 63.0 & 45.2 \\
        FCAF3D~\cite{rukhovich2021fcaf3d} & - & 71.5 & 57.3 & 64.2 & 48.9 \\
        CAGroup3D~\cite{wang2022cagroup3d} & - & 75.1 & 61.3 & 66.8 & 50.2 \\
        \midrule
        %OcCo\cite{wang2020unsupervised} & 59.8 & 37.9 & 59.6 & 34.8 \\
        STRL~\cite{huang2021spatio}& \checkmark & 59.5 & 38.4 & 58.2 & 35.0 \\
        RandomRooms~\cite{rao2021randomrooms}& \checkmark & 61.3 & 36.2 & 59.2 & 35.4 \\
        PointContrast~\cite{xie2020pointcontrast}& \checkmark & 59.2 & 38.0 & 57.5 & 34.8 \\
        DepthContrast~\cite{zhang2021self}& \checkmark & 62.1 & 39.1 & 60.4 & 35.4 \\
        Point-M2AE~\cite{zhang2022point}& \checkmark & 66.3 & 48.3 & - & - \\
        %DepthContrast($3\times$; \text{both}) & 64.0 & 42.9 \\
        \rowcolor{gray!20} MVNet + VoteNet & \checkmark & - & - & - & - \\
        \rowcolor{gray!20} MVNet + CAGroup3D & \checkmark & - & - & - & -\\
        \bottomrule
    \end{tabular}
\vspace{-4mm}
\end{table*}

==> tables/detection_spv.tex <==
\begin{table*}[t]
\centering
\setlength\tabcolsep{9pt}% 调整列间距
\begin{tabular}{lccccc}
    \toprule
     \multirow{2}{*}{Method} & \multicolumn{2}{c}{ScanNet} & \multicolumn{2}{c}{SUN RGB-D} \\
        \cmidrule(lr){2-3}   \cmidrule(lr){4-5}  & 
        mAP@0.25 & mAP@0.5 & mAP@0.25 & mAP@0.5 \\
        \midrule
        VoteNet~\cite{qi2019deep} & 58.6 & 33.5 & 57.7 & 32.9 \\
        3D-MPA~\cite{engelmann20203d}& 64.2 & 49.2 & - & - \\
        HGNet~\cite{chen2020hierarchical} & 61.3 & 34.4 & 61.6 & - \\
        MLCVNet~\cite{xie2020mlcvnet}& 64.5 & 41.4 & 59.8 & - \\
        %GSDN~\cite{gwak2020generative} & 62.8 & 34.8 & - & - \\
        H3DNet~\cite{zhang2020h3dnet} & 67.2 & 48.1 & 60.1 & 39.0 \\
        BRNet~\cite{cheng2021back}& 66.1 & 50.9 & 61.1 & 43.7 \\
        3DETR~\cite{misra2021end}& 65.0 & 47.0 & 59.1 & 32.7 \\
        VENet~\cite{xie2021venet} & 67.7 & - & 62.5 & 39.2 \\
        GroupFree~\cite{liu2021group}& 69.1 & 52.8 & 63.0 & 45.2 \\
        RGBNet~\cite{wang2022rbgnet} & 70.6 & 55.2 & 64.1 & 47.2 \\
        HyperDet3D~\cite{zheng2022hyperdet3d} & 70.9 & 57.2 & 63.5 & 47.3 \\
        FCAF3D~\cite{rukhovich2021fcaf3d} & 71.5 & 57.3 & 64.2 & 48.9 \\
        CAGroup3D~\cite{wang2022cagroup3d} & 75.1 & 61.3 & 66.8 & 50.2 \\
        \rowcolor{gray!20} MVNet + CAGroup3D & \textbf{75.5}\small{±0.3} & \textbf{61.8}\small{±0.3} & \textbf{67.2}\small{±0.2} & \textbf{51.1}\small{±0.3}\\
        \bottomrule
    \end{tabular}
\caption{\small{\textbf{Comparison of 3D object detection results with supervised methods.} We fine-tune our pre-trained model on ScanNetV2~\cite{dai2017scannet} and SUN-RGBD~\cite{song2015sun} datasets using CAGroup3D~\cite{wang2022cagroup3d}.}}
\label{tab:detection_spv}
\vspace{-4mm}
\end{table*}

==> tables/loss_ablation.tex <==
\begin{table}[h]
    \centering
    \caption{Ablation study on loss design.}
    \label{tab:ablation}
   \setlength\tabcolsep{6pt}% 调整列间距
    \begin{tabular}{cc|c}
        \toprule
        $\mathcal{L}_{2d}$ &$\mathcal{L}_m$ & ScanNet \\
        \midrule
        - & - & \\
         $\surd$ & - & \\
        -& $\surd$ &  \\
        $\surd$ & $\surd$ & \\
        \bottomrule
    \end{tabular}
\end{table}

==> tables/seg_det.tex <==
\begin{table*}[h]
\centering
\footnotesize
\setlength\tabcolsep{4pt}
\begin{tabular}{llllllllllll}
    \toprule
    \multirow{3}{*}{Method} & \multicolumn{5}{c}{Semantic Segmentation} & \multicolumn{4}{c}{3D Object Detection} \\
    & \multicolumn{3}{c}{S3DIS Area 5} & \multicolumn{3}{c}{S3DIS 6-Fold} & ScanNet \\
     \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-8} & OA & mIoU & OA & mIoU & mIoU & \\
    \midrule
    Jigsaw & 82.8 & - & 52.1 & 84.4 & - & 56.6& - \\
    OcCo & 85.9 & - & 55.4 & 85.1 & - & 58.5 & - \\
    STRL & -  & - & - & 84.2 & - & 57.1 & -\\ 
    PointContrast  &  - & 77.0 & 70.9 & - & - & - & 74.1 \\ 
    DepthContrast & -  & - & 70.6 & - & - & - & 71.2\\ 
    SceneContext &  - & - & 72.2 & - & - & - & 73.8 \\ 
    \rowcolor{gray!20} MVNet & \textbf{91.7}(91.6) & \textbf{79.5}(79.3) & \textbf{73.6}(73.3) & \textbf{91.8}(91.7) & \textbf{86.3}(86.2) & \textbf{78.3}(78.1) & \textbf{75.6}(75.2)\\
    
    %\rowcolor{gray!20}\textit{ Improvement} & \textcolor[rgb]{0,0.6,0}{+2.6} & \textcolor[rgb]{0,0.6,0}{+4.1} & \textcolor[rgb]{0,0.6,0}{+5.4} & \textcolor[rgb]{0,0.6,0}{+1.6} & \textcolor[rgb]{0,0.6,0}{+4.2} & \textcolor[rgb]{0,0.6,0}{+4.7} & \textcolor[rgb]{0,0.6,0}{+3.4}\\
    \bottomrule
\end{tabular}
\caption{\small{\textbf{Semantic segmentation results on S3DIS (evaluation by 6-Fold or in Area 5) and ScanNet V2.} We show Overall Accuracy (OA), mean Accuracy (mAcc), and mean Intersection over Union~(mIoU). Methods in the second section are self-supervised pre-training approaches. MVNet shows the average results of 3 runs.}}
\label{tab:semseg}
\end{table*}

==> tables/segmentation_3.tex <==
\begin{table*}[h]
\centering
\footnotesize
\setlength\tabcolsep{4pt}
\begin{tabular}{llllllll}
    \toprule
    \multirow{2}{*}{Method} & \multicolumn{3}{c}{S3DIS Area 5} & \multicolumn{3}{c}{S3DIS 6-Fold} & ScanNet \\
     \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-8} & OA & mAcc & mIoU & OA & mAcc & mIoU & mIoU \\
    \midrule
    %PointNet & 53.5 & 49.0 & 41.1 & 78.5 & 66.2 & 47.6 & - \\
    %PointCNN & 85.9 & 63.9 & 57.3 & 88.1 & 75.6 & 65.4 & 45.8 \\
    %SPGraph & 86.4 & 66.5 & 58.0 & 85.5 & 73.0 & 62.1 & - \\
    %PointWeb & 87.0 & 66.6 & 60.3 & 87.3 & 76.2 & 66.7 & - \\
    MinkowskiNet~\cite{choy20194d} & - & 71.7 & 65.4 & - & - & - & 67.9 \\
    PointTransformer~\cite{zhao2021point}~\cite{qian2022pointnext}  & 90.8 & 76.5 & 70.4 & 90.2 & 81.9 & 73.5 & 70.6\\
    PointNeXt~\cite{qian2022pointnext} & 90.7 & - & 70.8 & 90.3 & - & 74.9 & 71.5 \\
    Stratified Trans~\cite{lai2022stratified} & 91.5 & 78.1 & 72.0 & - & - & - & 74.3\\
    PointMetaBase~\cite{lin2022meta} & 91.4 & - & 72.0 & 91.3 & - & 77.0 & 72.8\\
    SR-UNet~\cite{xie2020pointcontrast} & 89.1 & 75.5 & 68.2 & 90.2 & 82.1 & 73.6 & 72.2 \\
    \midrule
    Jigsaw & 82.8 & - & 52.1 & 84.4 & - & 56.6& - \\
    OcCo & 85.9 & - & 55.4 & 85.1 & - & 58.5 & - \\
    STRL & -  & - & - & 84.2 & - & 57.1 & -\\ 
    PointContrast  &  - & 77.0 & 70.9 & - & - & - & 74.1 \\ 
    DepthContrast & -  & - & 70.6 & - & - & - & 71.2\\ 
    SceneContext &  - & - & 72.2 & - & - & - & 73.8 \\ 
    \rowcolor{gray!20} MVNet & \textbf{91.7}(91.6) & \textbf{79.5}(79.3) & \textbf{73.6}(73.3) & \textbf{91.8}(91.7) & \textbf{86.3}(86.2) & \textbf{78.3}(78.1) & \textbf{75.6}(75.2)\\
    
    %\rowcolor{gray!20}\textit{ Improvement} & \textcolor[rgb]{0,0.6,0}{+2.6} & \textcolor[rgb]{0,0.6,0}{+4.1} & \textcolor[rgb]{0,0.6,0}{+5.4} & \textcolor[rgb]{0,0.6,0}{+1.6} & \textcolor[rgb]{0,0.6,0}{+4.2} & \textcolor[rgb]{0,0.6,0}{+4.7} & \textcolor[rgb]{0,0.6,0}{+3.4}\\
    \bottomrule
\end{tabular}
\caption{\small{\textbf{Semantic segmentation results on S3DIS (evaluation by 6-Fold or in Area 5) and ScanNet V2.} We show Overall Accuracy (OA), mean Accuracy (mAcc), and mean Intersection over Union~(mIoU). Methods in the second section are self-supervised pre-training approaches. MVNet shows the average results of 3 runs.}}
\label{tab:semseg}
\end{table*}

==> tables/shape_task_backup.tex <==
\begin{table*}[t]
    \centering
    \footnotesize
    \resizebox{1.\linewidth}{!}{  
    \footnotesize
    \begin{tabular}{lcccccc}
        \toprule
        \multirow{2}{*}{Method} & Dataset & \multicolumn{3}{c}{ScanObjectNN} & \multicolumn{2}{c}{ShapeNetPart} \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-6} & OBJ-BG & OBJ-ONLY & PB-T50-RS & ins. mIoU & cls. mIoU \\
        \midrule
        Transformer$^{\dagger}$ ~\citep{yu2022point} & & 79.9 & 80.6 & 77.2 & 85.1 & 83.4 \\
        PointBERT~\citep{yu2022point} & & 87.4 & 88.1 & 83.1 & 85.6 & 84.1 \\
        MaskDiscr~\citep{Liu2022maskdis} & & 89.7 & 89.3 & 84.3 & 86.0 & 84.4 \\
        MaskSurfel~\citep{zhang2022masked} & & 91.2 & 89.2 & 85.7 & 86.1 & 84.4 \\
        ULIP~\citep{xue2023ulip} & 91.3 & & 89.4 & 86.4 & - & - \\
        PointMAE~\citep{pang2022masked} & & 90.0 & 88.3 & 85.2 & 86.1 & - \\
        \rowcolor{gray!20}MVNet-B & \textbf{91.5} & \textbf{90.1}  & \textbf{87.8} & \textbf{86.2} & \textbf{84.8} \\       
        \rowcolor{gray!20}MVNet-L & \textbf{95.2} & \textbf{94.2}  & \textbf{91.0} & \textbf{86.8} & \textbf{85.2} \\
        \bottomrule
    \end{tabular}
    }
    % \vspace{5pt}
    \vspace{-2mm}
    \caption{\footnotesize{\textbf{Performance comparison with other pre-training approaches on shape-level downstream tasks.} All the methods and MVNet-B use the same transformer backbone architecture. $^{\dagger}$ represents the \textit{from scratch} results and all other methods represent the \textit{fine-tuning} results using pretrained weights.}}
    \label{tab:shape-result}
    %\vspace{-3pt}
\end{table*}



==> tables/supervised_seg.tex <==
\begin{table*}[h]
\centering
\scriptsize
\setlength\tabcolsep{4pt}
\begin{tabular}{llllllll}
    \toprule
    \multirow{2}{*}{Method} & \multicolumn{3}{c}{S3DIS Area 5} & \multicolumn{3}{c}{S3DIS 6-Fold} & ScanNet \\
     \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-8} & OA & mAcc & mIoU & OA & mAcc & mIoU & mIoU \\
    \midrule
    PointNet~\citep{qi2017pointnet} & 53.5 & 49.0 & 41.1 & 78.5 & 66.2 & 47.6 & - \\
    PointCNN~\citep{li2018pointcnn} & 85.9 & 63.9 & 57.3 & 88.1 & 75.6 & 65.4 & 45.8 \\
    SPGraph~\citep{landrieu2018large} & 86.4 & 66.5 & 58.0 & 85.5 & 73.0 & 62.1 & - \\
    PointWeb~\citep{zhao2019pointweb} & 87.0 & 66.6 & 60.3 & 87.3 & 76.2 & 66.7 & - \\
    MinkowskiNet~\citep{choy20194d} & - & 71.7 & 65.4 & - & - & - & 67.9 \\
    Vision MVFusion~\citep{DBLP:conf/eccv/KunduYFRBFP20} & - & - & 65.4 & - & - & - & 74.6\\
    Voint Cloud~\citep{DBLP:conf/iclr/HamdiGG23} & - & - & 66.1 & - & - & - & 74.8 \\
    PointTransformer~\citep{zhao2021point}  & 90.8 & 76.5 & 70.4 & 90.2 & 81.9 & 73.5 & 70.6\\
    PointNeXt~\citep{qian2022pointnext} & 90.7 & - & 70.8 & 90.3 & - & 74.9 & 71.5 \\
    Stratified Trans~\citep{lai2022stratified} & 91.5 & 78.1 & 72.0 & - & - & - & 74.3\\
    PointMetaBase~\citep{lin2022meta} & 91.4 & - & 72.0 & 91.3 & - & 77.0 & 72.8\\
    SR-UNet~\citep{xie2020pointcontrast} & 89.1 & 75.5 & 68.2 & 90.2 & 82.1 & 73.6 & 72.2 \\
    \rowcolor{gray!20} MVNet & \textbf{91.7}(91.6) & \textbf{79.5}(79.3) & \textbf{73.8}(73.3) & \textbf{91.8}(91.7) & \textbf{86.3}(86.2) & \textbf{78.3}(78.1) & \textbf{75.6}(75.2)\\
    
    %\rowcolor{gray!20}\textit{ Improvement} & \textcolor[rgb]{0,0.6,0}{+2.6} & \textcolor[rgb]{0,0.6,0}{+4.1} & \textcolor[rgb]{0,0.6,0}{+5.4} & \textcolor[rgb]{0,0.6,0}{+1.6} & \textcolor[rgb]{0,0.6,0}{+4.2} & \textcolor[rgb]{0,0.6,0}{+4.7} & \textcolor[rgb]{0,0.6,0}{+3.4}\\
    \bottomrule
\end{tabular}
\caption{\small{\textbf{Comparison with supervised methods on S3DIS (evaluation by 6-Fold or in Area 5) and ScanNet V2.} The average result of 3 runs is given in parentheses.}}
\label{tab:supp-seg}
\end{table*}

==> tables/supp_fewshot.tex <==
\begin{table*}[t]
\centering
\setlength\tabcolsep{8pt}% 调整列间距
\scriptsize

\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{5-way}} & \multicolumn{2}{c}{\textbf{10-way}} \\
\cmidrule(lr){2-3}   \cmidrule(lr){4-5}
 & 10-shot & 20-shot & 10-shot & 20-shot \\
\hline
DGCNN$^{\dagger}$ & $31.6 \pm 2.8$ & $40.8 \pm 4.6$ & $19.9 \pm 2.1$ & $16.9 \pm 1.5$ \\
OcCo & $90.6 \pm 2.8$ & $92.5 \pm 1.9$ & $82.9 \pm 1.3$ & $86.5 \pm 2.2$ \\
CrossPoint & $92.5 \pm 3.0$ & $94.9 \pm 2.1$ & $83.6 \pm 5.3$ & $87.9 \pm 4.2$ \\
\hline
Transformer$^{\dagger}$ & $87.8 \pm 5.2$ & $93.3 \pm 4.3$ & $84.6 \pm 5.5$ & $89.4 \pm 6.3$ \\
OcCo & $94.0 \pm 3.6$ & $95.9 \pm 2.3$ & $89.4 \pm 5.1$ & $92.4 \pm 4.6$ \\
PointBERT & $94.6 \pm 3.1$ & $96.3 \pm 2.7$ & $91.0 \pm 5.4$ & $92.7 \pm 5.1$ \\
MaskDiscr & $95.0 \pm 3.7$ & $97.2 \pm 1.7$ & $91.4 \pm 4.0$ & $93.4 \pm 3.5$ \\
PointMAE & $96.3 \pm 2.5$ & $97.8 \pm 1.8$ & $92.6 \pm 4.1$ & $95.0 \pm 3.0$ \\
\rowcolor{gray!20} MVNet & $\pmb{97.2} \pm \pmb{1.8}$ & $\pmb{98.3} \pm \pmb{1.8}$ &  $\pmb{93.4} \pm \pmb{3.4}$ & $\pmb{95.8} \pm \pmb{3.2}$ \\
\bottomrule
\end{tabular}
\caption{\small{\textbf{Few-shot classification on ModelNet40.} We report the average accuracy (\%) and standard deviation (\%) of 10 independent experiments. $^{\dagger}$ represents the \textit{from scratch} results and all other methods represent the \textit{fine-tuning} results using pretrained weights.}}
\label{tab:mn_fewshot}

\end{table*}

==> tables/supp_label_eff.tex <==
\begin{table}[h]
\centering
\setlength\tabcolsep{8pt}
\begin{tabular}{lccc}
\toprule
\textbf{Method}            & \textbf{20\%} & \textbf{50\%} & \textbf{100\%} \\ 
\midrule
Train from scratch & 18.8          & 24.7          & 32.9           \\ 
PointContrast      & 24.5          & 29.2          & 37.5           \\ 
4DContrast         & 26.3          & 31.5          & 38.2           \\ 
MVNet              & \textbf{28.5} & \textbf{33.2} & \textbf{39.6}  \\ 
\bottomrule
\end{tabular}
\caption{\textbf{Label efficient training on SUN RGB-D object detection task.} We take the VoteNet as network architecture and compare our method with PointContrast and 4DContrast.}
\label{tab:supp-label}
\end{table}


==> tables/supp_shape_task.tex <==
\begin{table*}[t]
    \centering
    \resizebox{1.\linewidth}{!}{  
    \footnotesize
    \begin{tabular}{llccccc}
        \toprule
        \multirow{2}{*}{Method} & \multirow{2}{*}{Backbone} & \multicolumn{3}{c}{ScanObjectNN} & \multicolumn{2}{c}{ShapeNetPart} \\
        \cmidrule(lr){3-5} \cmidrule(lr){6-7} & & OBJ-BG & OBJ-ONLY & PB-T50-RS & ins. mIoU & cls. mIoU \\
        \midrule
        Jigsaw~\citep{sauder2019self} & DGCNN & 86.8 & 86.2 & 83.5 & 85.3 & - \\
        OcCo~\citep{wang2020unsupervised} & DGCNN & 88.2& 87.5 & 85.0 &  - \\
        CrossPoint~\citep{afham2022crosspoint} & DGCNN & - & - & 85.5 & 83.7\\
        ULIP~\citep{xue2023ulip} & Transformer & 91.3 & 89.4 & 86.4 & - & -\\
        ULIP~\citep{xue2023ulip} & PointMLP & 93.2 & 90.4 & 89.4 & - & -\\
        Point-M2AE~\citep{zhang2022point} & M2AE & 91.2 & 88.8 & 86.4 & 86.5 & 84.9\\
        I2P-MAE~\cite{zhang2023learning} & M2AE & 94.2 & 91.6 & 90.1 & \textbf{86.8} & \textbf{85.2}\\
        \rowcolor{gray!20}MVNet-L & Transformer & \textbf{95.2} & \textbf{94.2}  & \textbf{91.0} & \textbf{86.8} & \textbf{85.2} \\
        \bottomrule
    \end{tabular}
    }
    % \vspace{5pt}
    \vspace{-2mm}
    \caption{\small{\textbf{Performance comparison with pre-training approaches using different network backbones on shape-level downstream tasks.} }}
    \label{tab:supp-shape-result}
    %\vspace{-3pt}
\end{table*}


